Vapur: A Search Engine to Find Related Protein-Compound Pairs in COVID-19 Literature

Coronavirus Disease of 2019 (COVID-19) created dire consequences globally and triggered an intense scientific effort from different domains. The resulting publications created a huge text collection in which finding the studies related to a biomolecule of interest is challenging for general purpose search engines because the publications are rich in domain specific terminology. Here, we present Vapur: an online COVID-19 search engine specifically designed to find related protein - chemical pairs. Vapur is empowered with a relation-oriented inverted index that is able to retrieve and group studies for a query biomolecule with respect to its related entities. The inverted index of Vapur is automatically created with a BioNLP pipeline and integrated with an online user interface. The online interface is designed for the smooth traversal of the current literature by domain researchers and is publicly available at https://tabilab.cmpe.boun.edu.tr/vapur/ .

==> sections/abstract.tex <==
\begin{abstract}
    Coronavirus Disease of 2019 (COVID-19) created dire consequences globally and triggered an enormous scientific effort from different domains. Resulting publications formed a gigantic domain-specific collection of text in which finding studies on a biomolecule of interest is quite challenging for general purpose search engines due to terminology-rich characteristics of the publications. Here, we present Vapur, an online COVID-19 search engine specifically designed for finding related protein - chemical pairs. Vapur is empowered with a biochemically related entities-oriented inverted index in order to group studies relevant to a biomolecule with respect to its related entities. The inverted index of Vapur is automatically created with a BioNLP pipeline and integrated with an online user interface. The online interface is designed for the smooth traversal of the current literature and is publicly available at \url{https://tabilab.cmpe.boun.edu.tr/vapur/}.
\end{abstract}

==> sections/acknowledgements.tex <==
\section*{Acknowledgments}
TUBITAK-BIDEB 2211-A Scholarship Program (to A.K. and R.O.), and TUBA-GEBIP Award of the Turkish Science Academy (to A.O.) are gratefully acknowledged. E.O. is an employee of F. Hoffman - La Roche AG, Switzerland.

==> sections/appendices.tex <==
\section{Appendices}\label{sec:append}

\input{tables/annotation}

==> sections/conclusion.tex <==
\section{Conclusion}

We presented Vapur, a search engine with an emphasis on identifying protein - chemical relations in the COVID-19 domain. Vapur is the first search engine we know of that uses relation extraction to construct an inverted index of related biochemical entities. Thanks to the relation extraction model, Vapur can categorize relevant documents to a query with respect to related chemical entities and present organized search results. 

We evaluated the relation extraction model on ChemProt and observed that BioBERT outperforms English BERT on both development and test sets in terms of precision, recall, and F1-score. We further analyzed the model predictions and demonstrated the high specificity of the model at identifying contexts with biochemical relation information. 

Although we focused on COVID-19 in this work, our approach can find application in any biomedical domain with a different choice of database to index. We believe that domain-specific scientific search engines will gain more interest in the future since COVID-19 is unlikely to be the last global health crisis for human-kind. In order too promote the development and use of search engines to help coping with such difficult times, we make the underlying pipeline and Vapur available at \url{https://github.com/boun-tabi/vapur} and \url{https://tabilab.cmpe.boun.edu.tr/vapur/}, respectively.

==> sections/intro.tex <==
\section{Introduction}
Coronavirus Disease of 2019 (COVID-19) outbreak had severe impacts on human health all around the world since December 2019, but also triggered an exceptional amount of scientific work. As of September 2020, PubMed recorded over 45K articles \citep{litcovid} related to COVID-19 since its inception, including works on diagnosis \citep{dorche2020neurological}, drug repurposing \citep{gao2020repositioning}, and text-mining \citep{tarasova2020data}. As this tremendous literature keeps growing in the form of unstructured text, it also becomes more and more challenging for researchers to find the relevant information they need. Furthermore, the publications include named entities and chemical relations that challenge the general-purpose search engines. Therefore, it is of critical importance to build a search engine that can find relevant documents in this terminology-rich and domain-specific literature. 

Biomedical named entity recognition (NER) and relation extraction can be utilized to semantically structure the publications around the biochemically related entities. When named entities and their relations are extracted, a document can be expressed as a set of triplets of the form $(Entity1, Entity2, Relation)$. This formulation can be converted to a semantic index from the related entities to the publications in order to enable retrieving relevant documents to a query by entity and relation matching. If the same entities are referenced with different words (e.g. ACE2, Angiotensin-converting enzyme 2, Q9BYF1), we can use named entity normalization to identify different mentions of the same entity.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/workflow_5.png}
    \caption{The workflow of the pipeline behind Vapur. We first split the abstracts to sentences and use BERN to detect the entities in the text. We then identify the biochemical relations with the relation extraction model that we trained and reform the output as an inverted index of relations. Vapur leverages this inverted index to retrieve relevant publications to the query as categorized by related entities.}
    \label{fig:workflow}
\end{figure*}

In this work, we present Vapur, an online search engine to find related protein - compound pairs in the COVID-19 anthology. Vapur is empowered with a biochemical relation-based inverted index that is created through named entity recognition and relation extraction on CORD-19 abstracts \citep{wang2020cord}. In order to obtain the index, we first identify and normalize the named entities in the documents using a pre-trained model, BERN \citep{kim2019neural}. Afterward, we determine if the entity pairs in the same sentence are related to each other by training a binary relation extraction model on the ChemProt data set \cite{chemprot} and obtain a list of related entities for each abstract. We utilize these sets to construct an inverted index that maps related entities to the documents they are mentioned. We illustrate our pipeline in \Figref{fig:workflow} and present Vapur at \url{https://tabilab.cmpe.boun.edu.tr/vapur/}. We publicly share the code and models at \url{https://github.com/boun-tabi/vapur}.




==> sections/methods.tex <==
\section{Methods}
\input{tables/chemprot_relations}

\subsection{Data sets}\label{subsec:datasets}
    
\paragraph{CORD-19} We create an entity-oriented search engine for CORD-19 abstracts. CORD-19 is a regularly updated data set that contains studies related to COVID-19 and SARS-CoV-2. We use the CORD-19 snapshot of August 23, 2020, that contains $\approx$ 233K documents for which $\approx$ 143K unique abstracts are provided. Vapur indexes only these abstracts, but it is able to return the linked full-paper, as well.

\paragraph{ChemProt} We trained the binary relation extraction model using the ChemProt data set \citep{chemprot}, a curation of PubMed abstracts whose entities and relations are manually annotated. ChemProt consists of three file types: abstracts, entities, and relations. An abstract file contains a PubMed abstract ID and its text, whereas an entity file lists the chemicals and proteins in the linked abstract. Last, a relation file reports the relation type between entity pairs in the same sentence whose relation types can be inferred from the sentence. 

\input{tables/chemprot_stats}

The relations in ChemProt are categorized into 11, where the first 10 categories (CPR:0 to CPR:9) denote various types of biochemical relations, while the last category (CPR:10) is reserved for ``not relation" (i.e., the sentence explicitly states that there is no relation between the specified pair of entities). In this work, we focus on binary relation extraction, where we aim at determining whether a sentence states that there is a relation between the specified two entities or not. Therefore, we consider the entity pairs in the first 10 categories as positive samples. Likewise, since the sentences in the CPR:10 and the 
``Other" classes do not state that there is a relation between the corresponding pair of entities, we treat these two classes as the negative class. We describe each relation type and report their instance counts in the ChemProt data set in \Tabref{tab:chemprot_relations}. We also provide summary statistics for ChemProt in \Tabref{tab:chemprot_stats}.


\input{tables/preprocessed_sentences}

    
\subsection{Named Entity Recognition and Normalization}
We used BERN \citep{kim2019neural}, a neural NER architecture with an integrated normalizer that can perform in a multi-type setting, to identify and normalize the entities in CORD-19 abstracts. BERN is an ensemble of existing tools and models \citep{wei2015gnormplus, leaman2015tmchem, d2015sieve, wei2016beyond, wei2018tmvar, lee2020biobert} and outputs a set of IDs for each recognized entity, given a sentence.

In this study, we first tokenized the abstracts with GENIA \citep{kim2003genia} and identified 1.23M sentences. We used BERN to extract named entities and their IDs in these sentences and recognized 1.58M entities in total, in which 171K are chemicals and 318K are proteins. With normalization, we computed the number of unique chemicals and proteins as 20K and 70K, respectively.


\begin{figure}
    \centering
    \includegraphics[width=.475\textwidth]{figures/rel_extraction_architecture.pdf}
    \caption{Relation Extraction Model. Our model is composed of a BioBERT and a binary classification layer. We tokenize the input sentences by BioBERT tokenizer and enclose the biochemical entities with special tags ($<$e1$>$ and $<$e2$>$). BioBERT also adds \textit{CLS} and \textit{SEP} tags for fixed length-relation representation and sentence separation, respectively. We use BioBERT output of \textit{CLS} token to train our binary classifier.}
    \label{fig:model_architecture}
\end{figure}
\subsection{Relation Extraction}
We propose a BioBERT-based \citep{lee2020biobert} model 
to identify related entities in CORD-19 abstracts. To this end, we first preprocessed the sentences to explicitly encode the entities in the input and then fine-tuned BioBERT with the preprocessed sentences in ChemProt. We used the binary labels in Section \ref{subsec:datasets} as outputs.

\paragraph{Preprocessing:} We surrounded the named entities in the sentences with opening and closing tags to mark their location. We tagged chemicals with $<$e1$>$ and $<$/e1$>$ and proteins  with $<$e2$>$ and $<$/e2$>$ to encode entity type and location during training. When a sentence had multiple chemical - protein pairs, we considered each pair separately and created copies of the sentence with different tags. \Tabref{tab:preprocess} provides an example of input and its two preprocessed forms.




\paragraph{Model:} We used BioBERT to create a binary model that decides if two entities in the same sentence are related. We added a single-layer binary log-softmax classifier to BioBERT and trained the classifier with the inputs and outputs from the previous step. BioBERT creates a fixed-length relation representation for the starting tag \textit{CLS} and we used this representation to vectorize the sentences. We trained the binary classifier with cross-entropy loss where we considered the pairs in CPR:1-9 as positive and pairs in CPR:10 or no reported relation (i.e., the 
``Other" Type in Table \ref{tab:chemprot_relations}) as negative. \Figref{fig:model_architecture} illustrates our relation extraction model.

\paragraph{Experimental setup:} We conducted a hyper-parameter search with different optimizers, learning rates, and weight decays. We trained a model 10 times per parameter combination and selected the best one with respect to F-score on the development set. We found that the AdamW optimizer with a 0.00003 learning rate and 0.1 weight decay yields the best results. We selected the best setting for relation extraction and computed mean precision, recall, and F1-score as well as the standard deviation on the ChemProt development (dev) and test sets.


==> sections/related_work.tex <==
\section{Related Work}
Extracting information from the growing body of biomedical literature has become even more important with the explosion of scientific research. Efforts such as ChemProt \citep{chemprot} aim to promote research in this direction by presenting PubMed abstracts in which proteins, chemicals, and their relations are manually labeled. \citealp{liu2018attention} and \citealp{lim2018rnn} developed sequential models for chemical and protein relation extraction on ChemProt, while \citealp{peng2018chemical} used an ensemble of deep models with SVM. However, all these models depend on the named entities to be recognized beforehand.

Named entity recognition is a widely studied topic in biomedical text mining. Conditional Random Fields (CRF) was a popular approach in early biomedical NER studies \citep{leaman2015tmchem,  wei2015gnormplus, wei2018tmvar}  and with the rise of deep learning, sequential models were also integrated into the models \citep{sachan2018effective}. Recently, transformers-based NER models were popularized, including BERN \citep{kim2019neural} which is a state-of-the-art biomedical named entity recognition and normalization tool that builds on BioBERT \citep{lee2020biobert} to identify and normalize the entities in a sentence. BERN is adopted by recent general-domain biomedical text mining studies \citep{jang2019chimerdb} as well as a model to answer COVID-19 related questions based on CORD-19 \citep{lee2020answering}.

CORD-19 \citep{wang2020cord} is a data set comprising scientific publications related to COVID-19 and provided a valuable resource for text mining studies. \citealp{su2020caire} and \citealp{esteva2020co} developed question answering models with integrated information retrieval and summarization modules, while \citealp{wang2020comprehensive} focused on extracting the chemical entities in CORD-19 and presented an automatically annotated NER data set, CORD-NER. The entities in CORD-NER are annotated with multiple tools, but they are not normalized. Here, for the first time, we apply named entity normalization and relation extraction to CORD-19 in order to create a biochemical relation-aware search engine.


==> sections/results.tex <==
\section{Results and Discussion}

In this work, we built Vapur, a CORD-19 search engine empowered by text-mining. We applied named entity recognition, named entity normalization, and relation extraction to CORD-19 abstracts and automatically created an inverted index from related entities to publications. Therefore, the performance of the named entity extraction and relation extraction modules is critical to identify relevant works. Since BERN was already evaluated for named entity recognition and normalization on the biomedical domain \citep{kim2019neural}, here we focus on evaluating the relation extraction model.

We built the relation extraction model by fine-tuning a binary classifier on BioBERT and computed precision, recall, and F1-Score on the dev and test sets of ChemProt. We also fine-tuned the same classifier using English BERT based model and report the results in \Tabref{tab:chemprot_res}.

\Tabref{tab:chemprot_res} demonstrates that  BioBERT obtained higher scores in terms of all three metrics on both folds, indicating that BioBERT is superior to BERT as the pre-trained language model for relation extraction on ChemProt. We relate this with the fact that BioBERT is trained with a more domain-related text and BERT observed texts from a wider range.


\input{tables/chemprot_results}
\input{tables/chemprot_relation_group_metrics}
\input{tables/cord_relation_label_examples}  

We further investigated the performance of our relation extraction model by computing test accuracy for each chemical - protein relation (CPR) category and pairs with no assigned CPR label (i.e., Other). We observe that the relation extraction model achieved the highest accuracy in the \textit{Other} category, indicating that the model can successfully identify whether the context is sufficient to deduce a relation between the entities or not. We relate this with using BioBERT, which is a contextual model for relation representation. Context-awareness enables Vapur to eliminate the documents that mention the queried entity in irrelevant contexts and to retrieve a document only if it contains relation information for the query.


We analyzed 41 sample sentences that we predicted to be positive to discover the limitations of our methodology. Most of the incorrect relation labels are due to incorrect entity assignment by BERN. In some cases, parts of the protein sequence such as N-terminal, carboxyl terminal or residue names such as Asp238 are recognized as compound. \Tabref{tab:cord_19_examples} illustrates sample sentences with incorrectly labeled entities. More examples that are manually checked by a domain expert are presented on our GitHub page as an Appendix in the Readme file.
 
  

==> sections/vapur.tex <==
\section{Vapur}
\begin{figure*}
    \centering
    \includegraphics[width=.9\textwidth]{figures/vapur_ss_latest.png}
    \caption{A search scenario on Vapur. When \textit{Interleukin 1b} is entered as the query, Vapur lists the biochemically related compounds and displays the publications that mention the relation. Unique IDs of each chemical entity are displayed to help the user for further research.
    Similar proteins to \textit{Interleukin 1b} are also listed in order to let the user explore the index smoothly.}
    \label{fig:vapur_ss}
\end{figure*}
Vapur is an online search engine with a focus on finding related proteins and chemicals from CORD-19, a compilation of COVID-19 literature \citep{wang2020cord}. Vapur uses an inverted index that is constructed through mining the relations and entities in CORD-19  and is able to retrieve relevant documents to the queried biomolecule as categorized by the relation extraction model. Vapur's inverted index explicitly represents relations as related entity pairs and maps each relation to the documents in which the relation was mentioned.

We also interpret the relation-oriented index of Vapur as a graph to infer relations that cannot be inferred from the inverted index trivially. We construct a graph from the index such that the nodes represent biomolecules and the edges denote biochemical relations. The resulting graph satisfies the bipartiteness property, since we identify only the relations between proteins and chemicals during binary relation extraction. \Tabref{tab:graph_summary} demonstrates the summary statistics of this bipartite graph computed via networkx \citep{networkx}.


\input{tables/graph_summary}

We leverage the bipartite graph structure to identify similar biomolecules of the same type. We use SimRank \cite{jeh2002simrank} to compute pairwise node similarity and list the five most similar entities to the query. The aim is to encourage the user to explore the information in CORD-19 not only for exact matches to the query, but also similar entities.


The entities are represented as equivalence classes learned from named entity recognition and normalization steps. For instance,  ``Interleukin-1b" is represented as \{interleukin-1b, IL-1beta, IL1B, HGNC:5992, \dots, BERN:323737602\} in the index and Vapur retrieves related entities and relevant documents with a mention ``Interleukin-1b" even if the query is ``IL1B". The equivalence classes cover a wide range of mention types from free-text to BERN IDs to present a flexible search experience in terms of search terms.


Vapur represents each mention type as a string and adopts a 3-gram based matching algorithm to search the queried entity in its index. Given a query, Vapur first creates a multi-set of all 3-grams of the query and computes the similarity of this set to all 3-gram multi-sets of the mentions in the index, which are pre-computed. Vapur measures the similarity of the query to a mention by generalized Jaccard similarity:

$$
J(Q, M) = \frac{\sum_i min(Q_i, M_i)}{\sum_i max(Q_i, M_i)}
$$
\noindent where $Q$ and $M$ are query and mention vectors that store the count of each 3-gram. Generalized Jaccard similarity makes Vapur more robust while retrieving results for a mistyped query.


When the related entities are found and their related abstracts are retrieved, Vapur ranks the related entities by the number of times they are co-mentioned with the queried entity. Each entity is displayed with its most frequent mention alongside the links to the papers. \Figref{fig:vapur_ss} illustrates an example search scenario on Vapur, which is publicly available at \url{https://tabilab.cmpe.boun.edu.tr/vapur/}






==> tables/annotation.tex <==
\begin{longtable}{p{4.5cm} p{2.5cm} p{2.5cm} p{1.25cm} p{1.25cm} p{1.5cm}}
\toprule
\textbf{Sentence} & \textbf{Identified Chemical} & \textbf{Identified\phantom{xx} Protein} & \textbf{Relation Label} & \textbf{Chemical Label} &  \textbf{Protein Label} \\

\midrule
The N-terminal domain of the coronavirus nucleocapsid (N) protein adopts a fold resembling a right hand with a flexible, positively charged b-hairpin and a hydrophobic palm. &  N &  coronavirus nucleocapsid (N) protein &  0 &  0 &  1 \\ \hline
 Alanine substitution of either Arg-76 or Tyr-94 in the N-terminal domain of IBV N protein led to a significant decrease in its RNA-binding activity and a total loss of the infectivity of the viral RNA to Vero cells. &  Alanine &  IBV N protein &  0 &  0 &  1 \\ \hline
 Rat microsomal aldehyde dehydrogenase (msALDH) has no amino-terminal signal sequence, but instead it has a characteristic hydrophobic domain at the carboxyl terminus (Miyauehi, K., R. &  carboxyl &  msALDH &  0 &  0 &  1 \\ \hline
 The IMPDH inhibitor merimepodib (MMPD) is an investigational antiviral drug that acts as a noncompetitive inhibitor of IMPDH. &  merimepodib &  IMPDH &  1 &  1 &  1 \\ \hline
 EMA/PMA treatments significantly decreased amplifiable hg/cont and significantly increased the number of PVDA positive probes and their signal intensity compared to untreated spiked lung samples. &  EMA &  hg/cont &  0 &  1 &  0 \\ \hline
 EMA/PMA treatments significantly decreased amplifiable hg/cont and significantly increased the number of PVDA positive probes and their signal intensity compared to untreated spiked lung samples. &  PMA &  hg/cont &  0 &  1 &  0 \\ \hline
 Thus, EMA/PMA treatments offer a new approach to lower the amplifiable hg/cont in clinical samples and increase the success of PVDA and HTS to identify viruses. &  EMA &  hg/cont &  0 &  1 &  0 \\ \hline
 A role for glycosylation in cell-surface tetherin expression is supported by tunicamycin treatment, which inhibits the first step of N-linked glycosylation and impairs both cell-surface expression and antiviral activity. &  tunicamycin &  tetherin &  1 &  1 &  1 \\ \hline
 The effects of cholesterol depletion and PI3K/AKT signaling pathway activation during S. agalactiae-human umbilical vein endothelial cells (HUVEC) interaction were analysed by pre-treatment with methyl-$\beta$-cyclodextrin (M$\beta$ CD) or LY294002 inhibitors, immunofluorescence and immunoblot analysis. &  MbCD &  PI3K &  1 &  1 &  1 \\ \hline
 Inhibition of complex-type glycosylation with kifunensine, an inhibitor of the oligosaccharide processing enzyme mannosidase 1, had no effect on either the cell-surface expression or antiviral activity of tetherin. &  kifunensine &  oligosaccharide processing enzyme mannosidase 1 &  1 &  1 &  1 \\ \hline
 Conversely, results from cell-based small molecule screening studies have shown that the antibiotic hexachlorophene can down-regulate b-catenin in colon cancer cells. &  hexachlorophene &  b-catenin &  1 &  1 &  1 \\ \hline
 The CT of tetherin contains an "STS" sequence that is implicated in ubiquitylation, and a highly-conserved tyrosine-based motif, "YxxY", that is essential for clathrin-dependent endocytosis of tetherin, and activation of nuclear factor-$\kappa$B (NF-$\kappa$B) [16] [17] [18] [19] . &  tyrosine &  tetherin &  0 &  0 &  1 \\ \hline
 Here we report that hexachlorophene also counteracts the elevated bcatenin levels in EBV-infected B lymphomas. &  hexachlorophene &  bcatenin &  1 &  1 &  1 \\ \hline \hline
 Our results suggest that Siah-1 is targeted by both LMP-1 and hexachlorophene with opposite effects. &  hexachlorophene &  Siah-1 &  1 &  1 &  1 \\ \hline
 The hexachlorophene modulation of Siah-1 and b-catenin is independent of p53 and results in reduced expression of cyclin-D1 and c-Myc (target genes of b-catenin), leading to the growth arrest of B lymphoma cells. &  hexachlorophene &  Siah-1 &  1 &  1 &  1 \\ \hline
 Alanine substitution of either Arg-76 or Tyr-94 in the N-terminal domain of IBV N protein led to a significant decrease in its RNA-binding activity and a total loss of the infectivity of the viral RNA to Vero cells. &  Alanine &  IBV N protein &  0 &  0 &  1 \\ \hline
 Rat microsomal aldehyde dehydrogenase (msALDH) has no amino-terminal signal sequence, but instead it has a characteristic hydrophobic domain at the carboxyl terminus (Miyauehi, K., R. &  carboxyl &  Rat microsomal aldehyde dehydrogenase &  0 &  0 &  1 \\ \hline
 Also, the protease Factor Xa, a target of Ben-HCl abundantly expressed in infected cells, was able to cleave the recombinant and pseudoviral S protein into S1 and S2 subunits, and the cleavage was inhibited by Ben-HCl. &  Ben &  protease Factor Xa &  0 &  0 &  1 \\ \hline
 Since the 3a protein forms ion channels, we were interested to see any conformational changes occurring in the Cyot3a upon calcium binding, using fluorescence spectroscopy and circular dichroism. &  calcium &  3a protein &  1 &  1 &  1 \\ \hline
 These studies clearly indicate a significant change in the conformation of the Cyto3a protein after binding with calcium. &  calcium &  Cyto3a protein &  1 &  1 &  1 \\ \hline
 Our results strongly suggest that the cytoplasmic domain of the 3a protein of SARS-CoV binds calcium in vitro, causing a change in protein conformation. &  calcium &  3a protein &  1 &  1 &  1 \\ \hline
 Further, the drug hexamethylene amiloride (HMA), but not amiloride, inhibited in vitro ion channel activity of some synthetic coronavirus E proteins, and also viral replication. &  hexamethylene amiloride &  synthetic coronavirus E proteins &  1 &  1 &  1 \\ \hline
 The high prevalence of variants in the G6PD gene found in this analysis suggests that it may be a significant interaction factor in clinical trials of chloroquine and hydrochloroquine for treatment of COVID-19 in Africans. &  chloroquine &  G6PD gene &  1 &  1 &  1 \\ \hline
 In an effort to circumvent resistance to rapamycin -an mTOR inhibitor -we searched for novel rapamycindownstream-targets that may be key players in the response of cancer cells to therapy. &  rapamycin &  mTOR &  1 &  1 &  1 \\ \hline
 We found that rapamycin, at nM concentrations, increased phosphorylation of eukaryotic initiation factor (eIF) 2a in rapamycin-sensitive and estrogen-dependent MCF-7 cells, but had only a minimal effect on eIF2a phosphorylation in the rapamycininsensitive triple-negative MDA-MB-231 cells. &  rapamycin &  eukaryotic initiation factor (eIF) 2a &  1 &  1 &  1 \\ \hline
 Addition of salubrinal -an inhibitor of eIF2a dephosphorylationdecreased expression of a surface marker associated with capacity for self renewal, increased senescence and induced clonogenic cell death, suggesting that excessive phosphorylation of eIF2a is detrimental to the cells' survival. &  salubrinal &  eIF2a dephosphorylationdecreased &  1 &  1 &  1 \\ \hline
 Treating cells with salubrinal enhanced radiation-induced increase in eIF2a phosphorylation and clonogenic death and showed that irradiated cells are more sensitive to increased eIF2a phosphorylation than non-irradiated ones. &  salubrinal &  eIF2a &  1 &  1 &  1 \\ \hline
 Similar to salubrinal -the phosphomimetic eIF2a variant -S51D -increased sensitivity to radiation, and both abrogated radiation-induced increase in breast cancer type 1 susceptibility gene, thus implicating enhanced phosphorylation of eIF2a in modulation of DNA repair. &  salubrinal &  eIF2a variant &  1 &  1 &  1 \\ \hline
 In addition to its effect on radiation, salubrinal enhanced eIF2a phosphorylation and clonogenic death in response to the histone deacetylase inhibitor -vorinostat. &  salubrinal &  eIF2a &  1 &  1 &  1 \\ \hline
 Finally, the catalytic competitive inhibitor of mTOR -Ku-0063794 -increased phosphorylation of eIF2a demonstrating further the involvement of mTOR activity in modulating eIF2a phosphorylation. &  Ku-0063794 &  mTOR &  1 &  1 &  1 \\ \hline
 Moreover, glycyrrhizin treatment still enhanced IFN-$\gamma$ and reduced IL-4 levels in glycyrrhizin-treated mice. &  glycyrrhizin &  IFN-g &  1 &  1 &  1 \\ \hline
 While determining the 5' ends of C. elegans actin mRNAs, we have discovered a 22 nucleotide spliced leader sequence. &  nucleotide &  C. elegans actin mRNAs &  0 &  0 &  0 \\ \hline
 The actin mRNA leader sequence is identical to the first 22 nucleotides of a novel 100 nucleotide RNA transcribed adjacent, and in the opposite orientation, to the 5S ribosomal gene. &  nucleotides &  actin mRNA leader sequence &  0 &  0 &  0 \\ \hline
 The evidence suggests that the actln mRNA leader sequence is acquired from this novel nucleotide transcript by an intermolecular frans-splicing mechanism. &  nucleotide &  actln mRNA leader sequence &  0 &  0 &  0 \\ \hline
 We found that the aspartic acid at position 95, previously believed to be required for binding of PSGs to cells, is not required for PSG1 activity but that the amino acids implicated in the formation of a salt bridge within the N-domain are essential for PSG1 function. &  aspartic acid &  PSGs &  0 &  0 &  1 \\ \hline
 In vitro expression of a construct containing the Lb gene fused to a portion of the VP4 and 3D genes demonstrated cis cleavage activity that could be blocked by the thiol protease inhibitor E-64. &  E-64 &  Lb gene &  1 &  1 &  1 \\ \hline
 In contrast, conversion of LC3-I/LC3-II could be significantly inhibited by 4-PBA, an ER stress inhibitor, indicating that ORF3-induced autophagy is dependent on ER stress response. &  4-PBA &  LC3-I &  1 &  1 &  1 \\ \hline
 All the studied molecules could bind to the active site of the SARS-CoV-2 protease (PDB: 6Y84), out of which rutin (a natural compound) has the highest inhibitor efficiency among the 33 molecules studied, followed by ritonavir (control drug), emetine (anti-protozoal), hesperidin (a natural compound), lopinavir (control drug) and indinavir (anti-viral drug). &  rutin &  SARS-CoV-2 protease &  1 &  1 &  1 \\ \hline
 Using degenerate PCR primers complementary to the most conserved genome regions of adenoviruses, the complete nucleotide sequence of the penton base gene, and partial nucleotide sequences of the DNA polymerase, hexon, and pVII genes were obtained. &  nucleotide &  penton base gene &  0 &  0 &  1 \\ \hline
 Estradiol is connected with CD4+ T cell numbers and increases T-reg cell populations, affecting immune responses to infection. &  Estradiol &  CD4+ &  1 &  1 &  1 \\ \hline
 It is known that estradiol exerts a protective effect on endothelial function, activating the generation of nitric oxide (NO) via endothelial nitric oxide synthase. &  estradiol &  endothelial nitric oxide synthase &  1 &  1 &  1 \\
\bottomrule
\caption{Sample sentences from CORD-19 predicted by the proposed model to contain a biochemical relation. The results of the manual validation by a domain expert are reported. Chemical and protein columns denote the entities recognized by BERN; and chemical label and protein label columns report the expert label. The expert label is 1 if the recognition is correct and 0 otherwise. Similarly, the relation label is set to 1 if these entities are biochemically related.}
\end{longtable}

==> tables/chemprot_relation_group_metrics.tex <==
\begin{table}
    \centering
    \begin{tabular}{p{.15\textwidth} p{.25\textwidth}}
    \toprule  
    \textbf{Relation ID} & \textbf{Test Set Accuracy}\\
    \midrule
    CPR:1 & 0.661 $\pm$ 0.053\\
    CPR:2 & 0.667 $\pm$ 0.043\\
    CPR:3 & 0.855 $\pm$ 0.015\\
    CPR:4 & 0.874 $\pm$ 0.027\\
    CPR:5 & 0.850 $\pm$ 0.045\\
    CPR:6 & 0.856 $\pm$ 0.050\\
    CPR:7 & 0.890 $\pm$ 0.044\\
    CPR:8 & 0.550 $\pm$ 0.066\\
    CPR:9 & 0.617 $\pm$ 0.060\\
    CPR:10 & 0.828 $\pm$ 0.053\\
    \textit{Other} & 0.892 $\pm$ 0.020\\
    \bottomrule
    \\
    \end{tabular}

\caption{Test performance of the relation extraction model by CPR label. We used the best model trained with 10 random seeds to predict test set pairs and report mean and standard deviation of the test accuracy by label. The results display that the relation extraction model is the most successful at the \textit{Other} category, indicating its high context-awareness.
}
    \label{tab:chemprot_results_by_label}
\end{table}

==> tables/chemprot_relations.tex <==
\begin{table*}
    \centering
    \begin{tabular}{llllll}
    \toprule
    \begin{tabular}{@{}l@{}}\textbf{Relation} \\ \textbf{ID}\end{tabular}  & \textbf{Description} & \begin{tabular}{@{}l@{}}\textbf{Train} \\ \textbf{Count}\end{tabular} & \begin{tabular}{@{}l@{}}\textbf{Dev} \\ \textbf{Count}\end{tabular} & \begin{tabular}{@{}l@{}}\textbf{Test} \\ \textbf{Count}\end{tabular} & \begin{tabular}{@{}l@{}}\textbf{Binary} \\ \textbf{Label}\end{tabular} \\
        \midrule
        CPR:0 &  \textit{No description provided by ChemProt} & 1 & 2 & 0 & 1\\
        CPR:1 &  Part of & 308 & 153 & 215  & 1\\
        CPR:2 &  Regulator / Direct Regulator / Indirect regulator & 1652 & 780 & 1743 & 1 \\
        CPR:3 &  Upregulator /  Activator/ Indirect upregulator & 777 & 552 & 667 & 1\\
        CPR:4 &  Downregulator / Inhibitor / Indirect Downregulator & 2260 & 1103 & 1667 & 1 \\
        CPR:5 &  Agonist /  Agonist activator / Agonist inhibitor & 173 & 116 & 198 & 1\\
        CPR:6 &  Antagonist & 235 & 199 & 293 & 1 \\
        CPR:7 &  Modulator  / Modulator Activator / Modulator inhibitor & 29 & 19 & 25 & 1\\
        CPR:8 &  Cofactor & 34 & 2 & 25 & 1 \\
        CPR:9 &  Substrate / Product of / Substrate product of & 727 & 457 & 644 & 1\\
        CPR:10 &  Not relation & 241 & 175 & 267 & 0\\
        \textit{Other} & \textit{No relation information between entities in this context}& 11664 & 7780 & 9987 & 0\\
    \bottomrule
    \end{tabular}
    \caption{Chemical - Protein Relations (CPR) in ChemProt. The entity pairs are annotated with 11 different relations in ChemProt and we refer to pairs whose relation information cannot be inferred from the context as \textit{Other}. We report the instance count of each category and specify the label we assign to each category for binary relation extraction.}
    \label{tab:chemprot_relations}
\end{table*}


==> tables/chemprot_results.tex <==
\begin{table}
\centering
\resizebox{.5\textwidth}{!}{
\begin{tabular}{lllll}
\toprule \textbf{Fold} & \textbf{Model} & \textbf{Precision} &
\textbf{Recall} & \textbf{F1-Score}\\ \midrule

Dev & BERT  & 0.718$\pm$0.027 & 0.737$\pm$0.026  & 0.727$\pm$0.010  \\
& \textbf{BioBERT}  & \textbf{0.742$\pm$0.036} & \textbf{0.829$\pm$0.035}  & \textbf{0.782$\pm$0.012}  \\

\midrule
Test & BERT & 0.759$\pm$0.023 & 0.710$\pm$0.026 & 0.733$\pm$0.007\\
& \textbf{BioBERT} & \textbf{0.791$\pm$0.026} & \textbf{0.766$\pm$0.036} & \textbf{0.777$\pm$0.010}\\

\bottomrule
\\
\end{tabular}
}
\caption{BERT- and BioBERT-based fine-tuning results for binary relation extraction. We computed precision, recall, and F1 on the dev and test folds of ChemProt. The results show that BioBERT-based model outperforms BERT-based model in terms of all metrics on both folds.}
\label{tab:chemprot_res}
\end{table}

==> tables/chemprot_stats.tex <==
\begin{table}
\centering
\resizebox{.475\textwidth}{!}{
\begin{tabular}{llll}
\toprule
\textbf{Statistic}  & \textbf{Train} &   \textbf{Dev} & \textbf{Test} \\ \midrule
\# documents & 1020 & 612 & 800 \\
\# sentences & 18046   & 11294 & 15712\\
\# entities & 25752 & 15567 & 20828 \\
\# chemical mentions & 13017 & 8004 & 10810 \\
\# unique chemical entities & 3710 & 2517 & 3442 \\
\# protein mentions & 12735 & 7563 & 10018 \\
\# unique protein entities & 4610 & 3018 & 3757 \\
\# duplicate relations & 98 & 86 & 158 \\
\# positive labels & 6143 &	3339 &	5459 \\
\# negative labels & 11903 &	7955 &	10253 \\
\bottomrule
\end{tabular}
}
\caption{ChemProt summary statistics. We split abstracts to sentences via GENIA \citep{kim2003genia} and computed the statistics accordingly. We refer to relations in the same sentence with the same protein, chemical and relation type as duplicate relations and consider them only once during training. We observe that the \# of mentions is considerably higher than the \# of unique entities for both proteins and chemicals, emphasizing the need for normalization. In addition, negative entity pairs are significantly more frequent than the positive ones, but their distribution across the training, development, and test folds is similar.}
\label{tab:chemprot_stats}
\end{table}

==> tables/cord_relation_label_examples.tex <==
\begin{table*}
\resizebox{\textwidth}{!}{
\begin{tabular}{|p{13cm}|p{2.5cm}|}
\hline
\textbf{Sentence in CORD-19 }  & \textbf{Incorrectly\phantom{xxx} Labeled Entity}  \\ \hline

$<$e1$>$Alanine$<$/e1$>$ substitution of either Arg-76 or Tyr-94 in the N-terminal domain of $<$e2$>$IBV N protein$<$/e2$>$ led to a significant decrease in its RNA-binding activity and a total loss of the infectivity of the viral RNA to Vero cells.
& \textbf{Alanine}       
\\ \hline
$<$e2$>$Rat microsomal aldehyde dehydrogenase$<$/e2$>$ (msALDH) has no amino-terminal signal sequence, but instead it has a characteristic hydrophobic domain at the $<$e1$>$carboxyl$<$/e1$>$ terminus (Miyauehi, K., R. & \textbf{carboxyl} 
\\ \hline
Also, the $<$e2$>$protease Factor Xa$<$/e2$>$, a target of $<$e1$>$Ben$<$/e1$>$-HCl abundantly expressed in infected cells, was able to cleave the recombinant and pseudoviral S protein into S1 and S2 subunits, and the cleavage was inhibited by Ben-HCl. & \textbf{Ben}
\\ \hline

\end{tabular}
}
\caption{Sample sentences with incorrectly labeled entities. The entity types of \textit{Alanine, carboxyl}, and \textit{Ben} are incorrectly predicted as chemical by BERN during the named entity recognition step. Consequently, the relation extraction model incorrectly identified a biochemical relation. }
\label{tab:cord_19_examples}
\end{table*}

==> tables/graph_summary.tex <==
\begin{table}
\resizebox{.475\textwidth}{!}{
\begin{tabular}{ll}
\toprule
\textbf{Graph Property} & \textbf{Statistic} \\
\midrule
\# Nodes (Entities)                  & 12384 \\
\# Chemical Nodes                    & 5018  \\
\# Protein Nodes                     & 7366  \\
\# Edges (Relations)                 & 17657 \\
\# Connected Components              & 807   \\
\# Nodes in the Largest Component    & 10194  \\
\# Edges in the Largest Component    & 16226 \\
\# Diameter of the Largest Component & 18  \\
\bottomrule
\end{tabular}
}
\caption{Summary statistics for the bipartite graph of the inverted index. We observe that number of chemicals and proteins are comparable to each other and the number of relations is close to the number of nodes, indicating the sparsity. In addition, the graph is formed of 807 connected components but the largest one is significantly larger than the others.}
\label{tab:graph_summary}
\end{table}

==> tables/preprocessed_sentences.tex <==
\begin{table*}
\resizebox{\textwidth}{!}{
\begin{tabular}{|p{2.5cm}|p{13cm}|}
\hline
\textbf{Raw Sentence}             & EGFR  inhibitors currently under investigation include the small molecules gefitinib and erlotinib.                                    \\ \hline
\textbf{Preprocessed Form I}  & $<$e2$>$EGFR$<$/e2$>$  inhibitors currently under investigation include the small molecules $<$e1$>$gefitinib$<$/e1$>$ and erlotinib. \\ \hline
\textbf{Preprocessed Form II} & $<$e2$>$EGFR$<$/e2$>$  inhibitors currently under investigation include the small molecules gefitinib and $<$e1$>$erlotinib$<$/e1$>$. \\ \hline
\end{tabular}
}
\caption{An example of preprocessing. The raw sentence contains two chemicals (\textit{gefitinib}, \textit{erlotinib}) and one protein (EGFR), creating two protein - chemical pairs. Thus, we create two different forms of the sentence to encode each protein - chemical pair separately. We use $<$e1$>$ and $<$e2$>$ tags to enclose chemicals and proteins, respectively.}
\label{tab:preprocess}
\end{table*}
